ALBA : Reinforcement Learning for Video Object Segmentation

We consider the challenging problem of zero-shot video object segmentation (VOS). That is, segmenting and tracking multiple moving objects within a video fully automatically, without any manual initialization. We treat this as a grouping problem by exploiting object proposals and making a joint inference about grouping over both space and time. We propose a network architecture for tractably performing proposal selection and joint grouping. Crucially, we then show how to train this network with reinforcement learning so that it learns to perform the optimal non-myopic sequence of grouping decisions to segment the whole video. Unlike standard supervised techniques, this also enables us to directly optimize for the non-differentiable overlap-based metrics used to evaluate VOS. We show that the proposed method, which we call ALBA outperforms the previous stateof-the-art on three benchmarks: DAVIS 2017 [2], FBMS [20] and Youtube-VOS [27].

==> literature_summary.tex <==
FSEG
- Setting: ZS/Unsupervised moving object segmentation?
- Two stream conv architecture. 
- Pixel-wise classification of moving object.
- IID frame processing. 
- Training: Fully supervised based on ground-truth.
- Angle: Two stream makes things better.

LVO Memory
- Setting: ZS/Unsupervised moving object segmentation?
- Two stream architecture
    - Pre-trained & fixed DeepLAB + MPNet. 
- Pixel-wise CrossEntropy classification of moving object. 
- Memory via a hidden layer ConvGRU.
- Training: Fully supervised based on ground-truth.
- Angle: Memory makes things better.

OSVOS without Temporal (Hard to follow from quick skim).
- Setting: One-shot instance segmentation. 
- Use both end-to-end FCN & proposal generator. 
- Pixel-wise cross-entorpy classification. 
- IID frame processing.
- Training: Fine-tune from info in start frame.
- Angle: (1) Memory free is more robust to occlusion. (2) Easier to parallelize.

Anchor Diffusion: ICCV'19
- Setting: U-VOS. Davis'16.
- FCN pixel classifier. 
- ~= IID Frame processing.
- Training: On pairs: BCE training of anchor & query frames.
- Test time: Anchor computed once & re-used.
- Angle: (1) Memory free more robust. (2) Performance tends to degrade over time in sequential methods. Make it always use first frame as reference "memory" to avoid this. 

CosNet: CVPR'19
- Setting: U-VOS. Davis'16. YTO.
- FCN pixel classifier (deeplab based).
- ~= IID frame processing. 
- Training: On multiple pairs: BCE training of random pair using co-attention. 
- Testing: For each frame to segment, sample multiple support pairs to process along with it and exploit the co-attention.
- Angle: (1) Non-sequential more robust, more "augmentation". (2) But pairwise attention still shares knowledge. (3) Only end-to-end muli-frame model. Others are either single frame end-to-end, or multi-frame non-E2E.

RVOS: 
- Setting: U-Vos. Davis'17. Youtube-VOS. 
- FCN. ResNet Encoder. SpatioTemporal ConvLSTM. 
- Training: Pixel classification cross-entropy.
- Angle: Exploit both spatial and temporal knowledge. 

VIS: 
- Setting: VIS. Youtube-VIS.
- Modify MaskRCNN to have a tracking head that associates current proposal to one of the previously detected proposals in last frame, or create new object.
- Training: Supervised frame-wise & box/mask-wise training.

AGNN: 
- Setting: VOs. Davis'17.
- Jointly process all frames within sequence by using GNN. 
- Training: IID per frame. Pixel-wise cross-entropy. 
- Some use of proposals to get a shor list of potential pixels. But not grouping based.

MHPVOS:
- Setting: Semi-supervised VOS. 
- Training: Use deeplab/maskrcnn. Hand-crafted MHT-style algorithm to stitch. 

DMMNet
- Setting: Unsupervised VOS. 
- Use MaskRCNN. Differentiable Hungarian to stitch over time.
- Training: Not clear how. Presumably pixel-wise?

-------- RL METHODS -------------
Reinforcement cutting-agent learning for video object segmentation: 
- Setting: Semi-supervised
- Action space: Move boundingbox left/right/up/down + expand/shrink context box.
- “CPN” Policy Net: Finds the bounding box of the object, tracking style.
- “CEN” Segmentation Net: Segments the object within the box.
    - It seems that CEN is trained supervised and CPN by RL?
- I think it's Davis'16. Single object only?

Adaptive ROI Generation for Video Object Segmentation Using
Reinforcement Learning ( https://arxiv.org/pdf/1909.12482.pdf)
- Single object. Semi-supervised. Unpublished.

MASK-RL: Multiagent Video Object Segmentation
Framework Through Reinforcement Learning
- This is a TNNLS preprint that claims to be doing SS-VOS & U-VOS. Very confusing. 
- Hopefully we can slide with ignoring this.
-------- RL METHODS -------------


Notes:
- VIS vs VOS. VIS needs to classify objects as well, apparently (yang2019vis).

